Optimized Video Streaming over Cloud: A Stall-Quality Trade-off

As video-streaming services have expanded and improved, cloud-based video has evolved into a necessary feature of any successful business for reaching internal and external audiences. In this paper, video streaming over distributed storage is considered where the video segments are encoded using an erasure code for better reliability. There are multiple parallel streams between each server and the edge router. For each client request, we need to determine the subset of servers to get the data, as well as one of the parallel stream from each chosen server. In order to have this scheduling, this paper proposes a two-stage probabilistic scheduling. The selection of video quality is also chosen with a certain probability distribution. With these parameters, the playback time of video segments is determined by characterizing the download time of each coded chunk for each video segment. Using the playback times, a bound on the moment generating function of the stall duration is used to bound the mean stall duration. Based on this, we formulate an optimization problem to jointly optimize the convex combination of mean stall duration and average video quality for all requests, where the two-stage probabilistic scheduling, probabilistic video quality selection, bandwidth split among parallel streams, and auxiliary bound parameters can be chosen. This non-convex problem is solved using an efficient iterative algorithm. Evaluation results show significant improvement in QoE metrics for cloud-based video as compared to the considered baselines.

==> sec_00_abstract.tex <==
\begin{abstract}

As video-streaming services have expanded and improved, cloud-based video has evolved into a necessary feature of any successful business for reaching internal and external audiences. In this paper, video streaming over distributed storage is considered where the video segments are encoded using an erasure code for better reliability. There are multiple parallel connections between each server and the edge router. For each client request, a subset of servers as well as one of the parallel connections is needed to be determined to get the video. In order to have this scheduling, this paper proposes a two-stage probabilistic scheduling. Further, the selection of video quality is also chosen with a certain probability distribution. With these parameters, the playback time of video segments is determined by characterizing the download time of each coded chunk for each video segment. Using the playback times, a bound on the moment generating function on the stall duration is used to bound the mean stall duration. Based on this, we  formulate an optimization problem to jointly optimize the convex combination of mean stall duration and average video quality for  all requests, where the two-stage probabilistic scheduling, probabilistic video quality selection, bandwidth split among parallel connections, and auxiliary bound parameters can be chosen. This non-convex problem  is solved using an efficient iterative algorithm.  Numerical results show significant improvement in QoE metrics for cloud-based video as compared to the considered baselines.


%, and hence, being the first work to the best of our knowledge that considers video streaming over erasure-coded distributed cloud systems. For a selected quality, the playback time of video segments is determined by characterizing the download time of each coded chunk for each video segment. Then,   using the playback times, a bound on the moment generating function on the stall duration is used to bound the mean stall duration.  The weighted average quality of the streamed video and the mean stall duration are crucial  quality of experience (QoE) measures for the end users.  Thus, based on these metrics, we formulate an optimization problem to jointly optimize the convex combination of both the QoE metrics averaged over all requests over the access of the video content, the allocated bandwidth among the different queues and the quality of the streamed quality. The non-convex problem  is solved using an efficient iterative algorithm.  Numerical results show significant improvement in QoE metrics for cloud-based video as compared to the considered baselines.
\end{abstract}

==> sec_5_NumericalResults2.tex <==
\section{Numerical Results}\label{sec:num}
In this section, we evaluate our proposed  algorithm for optimization of mean and tail probability of stall duration and show the effect of the trade-off of parameter $\theta$. We first study the two extremes where only either mean stall duration objective or tail stall duration probability is considered. Then, we show the tradeoff between the two QoE metrics based on the trade-off parameter $\theta$.

%how the impact of the tradeoff objective function varies with respect to the trade-off factor.  



\begin{table}[b]
{\caption{Storage Node Parameters Used in our Simulation (Shift $\beta=10msec$
and rate $\alpha$ in 1/s)}
}


\resizebox{.49\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Node 1}} & \multicolumn{1}{c}{\textbf{Node 2}} & \multicolumn{1}{c}{\textbf{Node 3}} & \multicolumn{1}{c}{\textbf{Node 4}} & \multicolumn{1}{c}{\textbf{Node 5}} & \multicolumn{1}{c}{\textbf{Node 6}}\tabularnewline
\hline 
{$\alpha_{j}$} & {$18.2298$} & {$24.0552$} & {$11.8750$} & {$17.0526$} & {$26.1912$} & {$23.9059$}\tabularnewline
\hline 
\end{tabular}}

\resizebox{.5\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Node 7}} & \multicolumn{1}{c}{\textbf{Node 8}} & \multicolumn{1}{c}{\textbf{Node 9}} & \multicolumn{1}{c}{\textbf{Node 10}} & \multicolumn{1}{c}{\textbf{Node 11}} & \multicolumn{1}{c}{\textbf{Node 12}}\tabularnewline
\hline 
{$\alpha_{j}$} & {$27.006$} & {$21.3812$} & {$9.9106$} & {$24.9589$} & {$26.5288$} & {$21.8067$}\tabularnewline
\hline 
\end{tabular}\label{tab:Storage-Nodes-Parameters}
}
\end{table}

\subsection{Numerical Setup}
 We simulate our algorithm in a distributed storage system of $m=12$ distributed nodes, where each video file uses an $(7,4)$ erasure code. We consider $r=1000$ files, whose sizes are generated based on Pareto distribution \cite{arnold2015pareto} with shape factor of $2$ and scale of $300$, respectively. Thus, the first $1000$ file-sizes that are less than 40 minutes are chosen.  We also assume that the chunk service time  follows a shifted-exponential distribution with rate $\alpha_{j}$ and shift $\beta_{j}$, whose values are shown in Table 2, which are generated at random and kept fixed for the experiments. Unless explicitly stated, the arrival rate for the first $500$ files is $0.002s^{-1}$ while for the next $500$ files is set to be $0.003s^{-1}$. Chunk size $\tau$ is set to be equal to $4$ s. When generating video files, the sizes of the video file sizes are rounded up to the multiple of $4$ sec. We note that a high load scenario is considered for the numerical results. In practice, the load will not be that high. However, higher load helps demonstrate the significant improvement in performance as compared to the lightly loaded scenarios where there are almost no stalls. In order to initialize our algorithm, we use a random placement of files on all the servers. Further, we set $\pi_{ij}=k/n$ on the placed servers with $t_{i}=0.01$ $\forall i$ and $j \in \mathcal{S}_{i}$. However, these choices of $\pi_{ij}$ and $t_{i}$ may not be feasible. Thus, we modify the initialization of  $\boldsymbol{\pi}$  to be closest norm feasible solution  given above values of $\boldsymbol{\mathcal{S}}$ and $\boldsymbol{t}$.  We  compare our proposed approach with three strategies:
 \begin{enumerate}[leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left]
\item {\em Random Placement, Optimized Access (RP-OA): }  In this strategy, the placement is chosen at random where any $n$  out of $m$ servers are chosen for each file, where each choice is equally likely. Given the random placement, the variables $\boldsymbol{t}$ and $\boldsymbol{\pi}$ are optimized using the Algorithm in Section \ref{sec:algo}, where $\boldsymbol{\mathcal{S}}$-optimization is not performed.

\item {\em Optimized Placement, Projected Equal Access (OP-PEA): }
The strategy utilizes $\boldsymbol{\pi}$, $\boldsymbol{t}$ and $\boldsymbol{\mathcal{S}}$ as mentioned in the setup. Then, alternating optimization over placement and $\boldsymbol{t}$ are performed using the proposed algorithm.

 %In this strategy, the placement is optimized while the access is chosen equally likely at the servers chosen. In order to do that, we perform an iterative algorithm as in Section \ref{sec:algo}, where the $\boldsymbol{\pi}$-optimization is replaced by taking $\pi_{ij}=k/n$ $\forall i$ and $j \in \mathcal{S}_{i}$ and projecting $\boldsymbol{\pi}$ to the feasible set by finding the closest norm feasible solution given above values of $\boldsymbol{\mathcal{S}}$ and $\boldsymbol{t}$.


\item {\em Random Placement, Projected Equal Access (RP-PEA): } In this strategy, the placement is chosen at random where any $n$  out of $m$ servers are chosen for each file, where each choice is equally likely. Further, we set $\pi_{ij}=k/n$ on the placed servers with $t_{i}=0.01$ $\forall i$ and $j \in \mathcal{S}_{i}$. We then modify the initialization of $\boldsymbol{\pi}$ to be closest norm feasible solution  given above values of $\boldsymbol{\mathcal{S}}$ and $\boldsymbol{t}$. Finally, an optimization over $\boldsymbol{t}$ is performed to the objective using Algorithm (\ref{alg:NOVA_Alg1}).


\end{enumerate} 
 
\begin{figure*}[htb]
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0in 0in 0in 0.0in, clip, width=\textwidth]{figs/convgstall2}
		%	\vspace{-.3in}
		\captionof{figure}{Convergence of mean stall duration.}
		\label{fig:ConvgMeanStall}
	\end{minipage}%
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 0.0in 0in, clip, width=\textwidth]{figs/stall_vs_rate2}
		%	\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different video arrival rates with different video lengths. }
		\label{fig:meanArrRateSameSize}
	\end{minipage}
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 0.0in 0in, clip,width=\textwidth]{figs/stall_vidSize}
		%		\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different video sizes considering  $\ell=3$.  }
		\label{fig:meanArrRateDiffSize}
	\end{minipage}
	%\vspace{-.2in}
	
	\vspace{-.1in}
\end{figure*}


\subsection{Mean Stall Duration optimization}
In this subsection, we focus only on minimizing the mean stall duration of all files by setting $\theta=1$, {\em i.e.}, stall duration tail probability is not considered.% in this part of the simulation.

\subsubsection*{Convergence of the Proposed Algorithm}
Figure \ref{fig:ConvgMeanStall} shows the convergence  of our proposed algorithm, which alternatively optimizes the mean stall duration of all files over scheduling probabilities $\boldsymbol{\pi}$, auxiliary variables $\boldsymbol{t}$, quality probabilities $\boldsymbol{b}$, and bandwidth allocation weights $\boldsymbol{w}$. We notice that for $r=1000$ video files of size 600 sec with $m=12$ storage nodes and six quality levels shown in \ref{tab:DataRates}, the mean stall duration converges to the optimal value within less than $300$ iterations.  


\subsubsection*{Effect of Arrival Rate} Figures \ref{fig:meanArrRateSameSize}  shows the effect of different video arrival rates on the mean stall duration for different-size video  whose lengths follow the Pareto-distributed described above.  We compare our proposed algorithm with the three baseline  policies and see that the proposed algorithm outperforms all baseline strategies for the QoE metric of mean stall duration. Thus, both access and bandwidth weights allocation of files are both important for the reduction of mean stall duration. We see that the mean stall duration increases with arrival rates. However, our approach still maintain low mean stall duration compared to the baselines.


%Intuitively, having optimized placement leads to less stall duration (for all policies) since video chunks are balanced across the different storage nodes. Hence, the possibility of congested bottleneck nodes reduces accordingly. While mean stall duration increases as arrival rate increases, our approach, unlike PEAP and BNW, does not explode  as others do (especially for optimized one). 

\subsubsection*{Effect of Video Size}
The effect of having different video sizes is also captured in Figure (\ref{fig:meanArrRateDiffSize}). Clearly, larger video sizes may incur more stalls compared to small ones as the chance of getting delayed chunks is increased. However, our proposed approach gives the lowest mean stall duration compared to the considered baselines.
%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_7_mean_stall_NoOfFiles_source.eps}
%\caption{Mean stall duration for different number of video files with different video sizes. \label{fig:meanStallNumFiles} }
%\end{figure}


\subsubsection*{Effect of the Number of Video Files}

Figure \ref{fig:meanStallNumFiles} demonstrates the impact of varying the number of video files from $200$ files to $1000$ files  on the mean stall duration, where the video lengths are generated according to Pareto distribution with the same parameter defined earlier (scale of 300, and shape of 2).  We note that the proposed optimization strategy effectively reduces the mean stall duration and outperforms the considered baseline strategies. Thus, joint optimization over all three variables $\boldsymbol{t}$,  $\boldsymbol{\pi}$,  $\boldsymbol{w}$, and  $\boldsymbol{b}$ helps reduce the mean stall duration significantly.


\subsection{Average Quality  Optimization}

In this subsection, we consider optimizing (magnifying) the quality of the streamed video by maximizing the quality probabilities, $\boldsymbol{b}$, by setting $0.5\leq\theta_{q}\leq1$
 in (\ref{eq:joint_otp_prob}).

\subsubsection*{Varying Quality factor parameter}
Figure \ref{fig:congStallDiffXvalues} 
 shows the average quality of the streamed videos versus the
stall factor $\theta_{s}$ for the selected set of algorithms. Apparently,
our proposed approach gives the highest quality as it aggressively
maximizes the quality over the stall duration, i.e., streaming the
larger videos by the highest possible probability. These results show
also the greedy behavior of our proposed approach as $\theta_{q}$  increases (or alternatively $\theta_{s}$ decreases) and clearly at $\theta_{q}=1$ (that is, $\theta_{s}=0$) our approach streams the video of the largest size and thus the average quality of the streamed video is
$\ell=6$, i.e., which is the highest possible quality. 


\begin{figure*}
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 0.0in 0in, clip, width=\textwidth]{figs/stall_NoOfVid}
%		\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different number of video files with different video lengths.}
		\label{fig:meanStallNumFiles} 
	\end{minipage}%
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 0.0in 0in, clip, width=\textwidth]{figs/qualty_vs_theta_q}
%		\vspace{-.3in}
		\captionof{figure}{ Average Streamed Quality versus quality factor $\theta_q$}
		\label{fig:congStallDiffXvalues}
	\end{minipage}
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0in 0in 0.1in 0in, clip,width=\textwidth]{figs/qlty_stall_vs_d}
%		\vspace{-.3in}
		\captionof{figure}{Average Video Quality and Mean Stall duration versus the number of virtual queues $d$}
		\label{fig:tailProbDiffX}
	\end{minipage}
%	\vspace{-.2in}

\vspace{-.15in}
\end{figure*}




%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_8_stallTail_vs_Num_iterations_source2.eps}
%\caption{Stall duration Tail Probability for different $x$. \label{fig:congStallDiffXvalues} }
%\end{figure}

%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_9_wieghtedLat_vs_x_comp_logy_source.eps}
%\caption{Stall duration tail probability for different $x$ (in seconds). \label{fig:tailProbDiffX} }
%\end{figure}
\subsubsection*{ Effect of the Number of the Virtual Queues $d$}
Figure \ref{fig:tailProbDiffX} plots the 
average of the streamed video quality and mean stall duration versus the number of virtual queses $d$. We vary the number of VQs from 5 to 30 with increment step of 5 and we set $\theta_q=1e-6$. We can see that the stall duration decreases as the number of VQs increases since more jobs can be handled simultaneously. We also observe that the proposed algorithm gives higher quality as $d$ increases which results from serving more than a job concurrently and allows for larger videos to be served. Hence, the proposed algorithm manages to significantly improve the two QoE metrics as $d$ increases.

%\begin{figure*}
%	\centering
%%	\begin{minipage}{.32\textwidth}
%%		\centering
%%		\includegraphics[trim=0in 0in 0.1in 0in, clip, width=\textwidth]{figs/tradeOff}
%%%		\vspace{-.3in}
%%		\captionof{figure}{Stall duration tail probability for different arrival rates for video files ($x=150$ s).}
%%		\label{fig:tailProbArrRate}
%%	\end{minipage}%
%%		\hspace{2mm}
%%		\begin{minipage}{.32\textwidth}
%%			\centering
%%		\includegraphics[trim=0in 0in 0.1in 0in, clip, width=\textwidth]{figs/convgstall2}
%%%		\vspace{-.3in}
%%		\captionof{figure}{Stall duration tail probability for varying number of video files ($x=150$ s).}
%%		\label{fig:Fig_9_stallLat_vs_NumOfFiles}
%%		\end{minipage}
%%		\hspace{2mm}
%		\begin{minipage}{.32\textwidth}
%			\centering
%			\includegraphics[trim=0in 0in 0.0in 0in, clip,width=\textwidth]{figs/tradeOff}
%	%		\vspace{-.3in}
%			\captionof{figure}{Tradeoff between mean stall duration and stall duration tail probability obtained by varying $\theta$.  }
%			\label{fig:tradeoff}
%		\end{minipage}
%	
%		\vspace{-.2in}
%\end{figure*}

\begin{figure}[t]
	\centering
%		\hspace{2mm}
		\begin{minipage}{.32\textwidth}
			\centering
			\includegraphics[trim=0in 0in 0.0in 0in, clip,width=\textwidth]{figs/tradeOff}
	%		\vspace{-.3in}
			\captionof{figure}{Tradeoff between mean stall duration and streamed video quality obtained by varying $\theta_s$.  }
			\label{fig:tradeoff}
		\end{minipage}
	
		\vspace{-.2in}
\end{figure}


\subsection{Tradeoff  between mean stall duration and video quality}


The preceding results show a trade off between the mean stall duration and
the streamed quality. In order to investigate such tradeoff, Figure \ref{fig:tradeoff} plots the average video quality versus the mean stall duration for different values of $\theta$ ranging from $\theta=10^{-5}$ to $\theta=10^{-7}$. This figure implies that a compromise between the two QoE metrics can be achieved by our proposed   streaming algorithm by setting the quality and stall factors ($\theta_q$ and $\theta_s$) to proper values. As expected, increasing $\theta_s$ will reduce the mean stall duration as higher priority is giving to minimize the stall over the quality. Thus, an efficient tradeoff point between the QoE metrics can be chosen based on the point on the curve that is appropriate for the clients.



==> sec_5_NumericalResultsCpy.tex <==
\section{Numerical Results}\label{sec:num}

In this section, we evaluate our proposed  algorithm for joint optimization of the mean stall duration and the average streamed video quality. 

%Further, we show the effect of the trade-off of the  parameter $\theta$. We study the two extremes where only either mean stall duration objective or video quality is considered. 

%Then, we show the tradeoff between the two QoE metrics based on the trade-off parameter $\theta$.

%how the impact of the tradeoff objective function varies with respect to the trade-off factor.  

{\scriptsize{}}
\begin{table}[b]
{\scriptsize{}\caption{{\small{}
The value of $\alpha_j/a_1$  used in the Numerical Results, where the units are 1/s.
\vspace{-.1in}
%For $1<\ell\leq10$, both $\beta_{j}^{(\ell)}$ and $\alpha_{j}^{(\ell)}$are scaled by $DR^{(\ell)}/DR^{(1)}$.
\label{tab:Storage-Nodes-Parameters}}}
}{\scriptsize \par}

{\scriptsize{}}%
\begin{tabular}{|c|>{\centering}p{2.53cc}|>{\centering}p{2.53cc}|c|c|c|}
\multicolumn{1}{>{\centering}p{2.53cc}}{{\scriptsize{}Node 1}} & \multicolumn{1}{>{\centering}p{2.53cc}}{{\scriptsize{}Node 2}} & \multicolumn{1}{>{\centering}p{2.53cc}}{{\scriptsize{}Node 3}} & \multicolumn{1}{c}{{\scriptsize{}Node 4}} & \multicolumn{1}{c}{{\scriptsize{}Node 5}} & \multicolumn{1}{c}{{\scriptsize{}Node 6}}\tabularnewline
\hline 
{\scriptsize{}$18.238$} & {\scriptsize{}$24.062$} & {\scriptsize{}$11.950$} & {\scriptsize{}$17.053$} & {\scriptsize{}$26.191$} & {\scriptsize{}$23.906$}\tabularnewline
\hline 
\end{tabular}{\scriptsize \par}

{\scriptsize{}}%
\begin{tabular}{|c|>{\centering}p{2.53cc}|>{\centering}p{2.53cc}|c|c|c|}
 \multicolumn{1}{>{\centering}p{2.53cc}}{{\scriptsize{}Node 7}} & \multicolumn{1}{>{\centering}p{2.53cc}}{{\scriptsize{}Node 8}} & \multicolumn{1}{>{\centering}p{2.53cc}}{{\scriptsize{}Node 9}} & \multicolumn{1}{c}{{\scriptsize{}Node 10}} & \multicolumn{1}{c}{{\scriptsize{}Node 11}} & \multicolumn{1}{c}{{\scriptsize{}Node 12}}\tabularnewline
\hline 
{\scriptsize{}$27.006$} & {\scriptsize{}$21.381$} & {\scriptsize{}$9.910$} & {\scriptsize{}$24.959$} & {\scriptsize{}$26.529$} & {\scriptsize{}$23.807$}\tabularnewline
\hline 
\end{tabular}{\scriptsize \par}
\vspace{-.15in}
\end{table}
{\scriptsize \par}


%\begin{table}[b]
%\caption{{\small{}Storage Node Parameters Used in our Simulation for $\ell=1$
%(Shift $\beta_{j}^{(1)}=10msec$ and rate $\alpha_{j}^{(1)}$ in 1/s).
%For $1<\ell\leq10$, both $\beta_{j}^{(\ell)}$ and $\alpha_{j}^{(\ell)}$
%are scaled by $DR^{(\ell)}/DR^{(1)}$.}}
%{\small{}}%
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{\small{}Node 1}} & \multicolumn{1}{c}{\textbf{\small{}Node 2}} & \multicolumn{1}{c}{\textbf{\small{}Node 3}} & \multicolumn{1}{c}{\textbf{\small{}Node 4}} & \multicolumn{1}{c}{\textbf{\small{}Node 5}} & \multicolumn{1}{c}{\textbf{\small{}Node 6}}\tabularnewline
%\hline 
%{\small{}$\alpha_{j}^{(1)}$} & {\small{}$18.2298$} & {\small{}$24.0552$} & {\small{}$11.8750$} & {\small{}$17.0526$} & {\small{}$26.1912$} & {\small{}$23.9059$}\tabularnewline
%\hline 
%\end{tabular}{\small \par}
%
%{\small{}}%
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{\small{}Node 7}} & \multicolumn{1}{c}{\textbf{\small{}Node 8}} & \multicolumn{1}{c}{\textbf{\small{}Node 9}} & \multicolumn{1}{c}{\textbf{\small{}Node 10}} & \multicolumn{1}{c}{\textbf{\small{}Node 11}} & \multicolumn{1}{c}{\textbf{\small{}Node 12}}\tabularnewline
%\hline 
%{\small{}$\alpha_{j}^{(1)}$} & {\small{}$27.006$} & {\small{}$21.3812$} & {\small{}$9.9106$} & {\small{}$24.9589$} & {\small{}$26.5288$} & {\small{}$21.8067$}\tabularnewline
%\hline 
%\end{tabular}\label{tab:Storage-Nodes-Parameters}
%\end{table}

\subsection{Parameter  Setup}
 We simulate our algorithm in a distributed storage system of $m=12$ distributed nodes, where each video file uses an $(7,4)$ erasure code. However, our model can be used for any given number of storage servers and for any erasure coding setting. We assume $d_j=20$ (unless otherwise explicitly stated) and $r=1000$ files, whose sizes are generated based on Pareto distribution \cite{arnold2015pareto} with shape factor of $2$ and scale of $300$, respectively. Since we assume that the file sizes are not heavy-tailed, the first $1000$ file-sizes that are less than 60 minutes are chosen.  We also assume that the chunk service time  follows a shifted-exponential distribution with rate $\alpha_{j}^{(\ell)}$ and shift $\beta_{j}^{(\ell)}$, given as \eqref{eq:alphabeta}. The value of $\beta_j a_1$ is chosen to be 10 ms, while the value of $\alpha_j/a_1$ is chosen as  in Table \ref{tab:Storage-Nodes-Parameters}. Unless explicitly stated, the arrival rate for the first $500$ files is $0.002s^{-1}$ while for the next $500$ files is set to be $0.003s^{-1}$. Chunk size $\tau$ is set to be equal to $4$ sec. When generating video files, the sizes of the video file sizes are rounded up to the multiple of $4$ sec. The data rates corresponding to each quality level is shown in Table \ref{tab:DataRates} \cite{svcParm015}. Thus, the different qualities $a_{\ell}$, $\ell = 1, \cdots, V$,  are $4s$ times the data rate in Table \ref{tab:DataRates}, where $V=6$. We use a random placement of files on 7 out of the 12 servers.  In order to initialize our algorithm, we assume uniform scheduling,  $q_{i,j}^{(\ell)}=k/n$ on the placed servers and $p_{j,\nu_j}^{(\ell)} = 1/d_j$. Further, we choose  $t_{i}=0.01$,  $b_{i, \ell}=1/V$, and $w_{j, \nu_j}=1/d_j $. However, these choices of the initial parameters may not be feasible. Thus, we modify the parameter initialization
 % $\boldsymbol{q}$  
 to be closest norm feasible solutions.
 
 
 
% To get the size of the video in  bytes, we multiply the size of the video in seconds by the data rate (DR) of each quality level. Thus, the possible choices of $a_{\ell}$ are $4s$ 
 
 
 
%  and for $\ell \neq1$, we used (xx) and (xx) to calculate the values of $\alpha_j^{(\ell)}$ and $\beta_j^{(\ell)}$,  respectively. %, which are generated at random and kept fixed for the experiments.

 \begin{table}[t]
\caption{{\small{}Data Rates (in $Mbps$) of the different quality levels.\label{tab:DataRates}}}
\vspace{-.15in}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline 
$\ell$ & 1 & 2 & 3 & 4 & 5 & 6\tabularnewline
\hline 
DR & $1.5$ & $2.75$ & $4.8$ & $7.8$ & $10.25$ & $12.5$\tabularnewline
\hline 
\end{tabular}
\vspace{-.1in}
\end{table}
%  given above values of $\boldsymbol{p}$, $\boldsymbol{b}$ , $\boldsymbol{w}$ and $\boldsymbol{t}$.  

\subsection{Baselines}
We  compare our proposed approach with six strategies, which are described as follows. 
 \begin{enumerate}
 
% the placement is chosen at random where any $n$  out of $m$ servers are chosen for each file, where each choice is equally likely. Given the random placement,

%1
%\item {\em Proposed Algorithm:} In this strategy, the joint scheduler is determined by the proposed solution that
%minimizes the convex combination of the weighted average quality and the mean stall duration, with
%respect to the five sets of variables: auxiliary variables $\boldsymbol{t}$, server access probabilities $\boldsymbol{q}$, VM selection probabilities $\boldsymbol{p}$, bandwidth allocation weights $\boldsymbol{w}$, and video quality probabilities $\boldsymbol{b}$.
%% are alternatively optimized using the Algorithm in Section \ref{sec:algo}.

%2
\item {\em Projected Equal Access, Optimized Quality Probabilities, Auxiliary variables and Bandwidth Wights (PEA-QTB):} Starting with the initial solution mentioned above, the problem in \eqref{eq:joint_otp_prob} is optimized over the choice of $\boldsymbol{t}$, $\boldsymbol{b}$, $\boldsymbol{w}$ and $\boldsymbol{p}$ (using Algorithms \ref{alg:NOVA_Alg1}, \ref{alg:NOVA_Alg3},  \ref{alg:NOVA_Alg4}, and
\ref{alg:NOVA_Alg5}, 
respectively)  using alternating minimization. Thus, the value of $q_{i,j}^{(\ell)}$ will be approximately close to $k/n$ for the servers on which the content is placed, indicating equal access of the $k$-out-of-$n$ servers. 

%In this strategy, the initialization is as mentioned above

%we set $q_{i,j}^{(\ell)}=k/n$ $\forall i, \ell, j$ on the placed servers. Then, we modify the initialization of $\boldsymbol{q}$ to be closest norm feasible solution  given the values of $\boldsymbol{p}$, $\boldsymbol{t}$, $\boldsymbol{b}$ and $\boldsymbol{w}$. Finally, an alternating optimization over , $\boldsymbol{t}$, $\boldsymbol{b}$, $\boldsymbol{w}$ and $\boldsymbol{p}$ is performed to the objective using Algorithms \ref{alg:NOVA_Alg1}, \ref{alg:NOVA_Alg3},  \ref{alg:NOVA_Alg4}, and \ref{alg:NOVA_Alg5},  respectively.



%3

\item {\em Projected Equal Bandwidth, Optimized Quality Probabilities, Auxiliary variables and Server Access (PEB-QTA):} Starting with the initial solution mentioned above, the problem in \eqref{eq:joint_otp_prob} is optimized over the choice of $\boldsymbol{q}$, $\boldsymbol{t}$, $\boldsymbol{b}$, and $\boldsymbol{p}$ (using Algorithms \ref{alg:NOVA_Alg1Pi}, \ref{alg:NOVA_Alg1},  \ref{alg:NOVA_Alg3}, and \ref{alg:NOVA_Alg5}, respectively) using alternating minimization. Thus, the bandwidth split $w_{j,\nu_j}$ will be  approximately $1/d_j$. 

%In this strategy, we set $w_{j,\nu_j} = 1/d_j, \, \forall j, \nu_j$.  Then, we modify this choice to be closest norm feasible solution  given the values of other sub-problems optimization parameters. Finally, an alternating optimization over $\boldsymbol{q}$, $\boldsymbol{t}$, $\boldsymbol{b}$, and $\boldsymbol{p}$ is performed to the objective using Algorithms \ref{alg:NOVA_Alg1Pi}, \ref{alg:NOVA_Alg1},  \ref{alg:NOVA_Alg3}, and \ref{alg:NOVA_Alg5}, respectively.


%% 4
\item {\em Projected Equal Quality, Optimized Bandwidth Wights, Auxiliary variables and Server Access (PEQ-BTA):} Starting with the initial solution mentioned above, the problem in \eqref{eq:joint_otp_prob} is optimized over the choice of $\boldsymbol{q}$, $\boldsymbol{t}$, $\boldsymbol{w}$, and $ \boldsymbol{p}$ (using Algorithms  \ref{alg:NOVA_Alg1Pi}, \ref{alg:NOVA_Alg1},  \ref{alg:NOVA_Alg4}, and \ref{alg:NOVA_Alg5}, respectively)  using alternating minimization. Thus, the quality assignment, $b_{i,\ell}$ will be approximately $1/V$. 


%In this strategy, we set $b_{i,\ell}=1/V,\, \forall i, \ell$ to be equal. Then, this choice is projected to be closest norm feasible solution. We then perform an alternating optimization over the remaining set of variables including $\boldsymbol{q}$, $\boldsymbol{t}$, $\boldsymbol{w}$, and $ \boldsymbol{p}$ using Algorithms  \ref{alg:NOVA_Alg1Pi}, \ref{alg:NOVA_Alg1},  \ref{alg:NOVA_Alg4}, and \ref{alg:NOVA_Alg5}, respectively.

%% 5
\item {\em (Projected Proportional Service-Rate, Optimized Quality, Auxiliary variables and Bandwidth Wights (PSP-QTB):} In the initialization, the access probabilities among the servers on which file $i$ is placed, is given as  $q_{i,j}^{(\ell)}=k_{i}\frac{\mu_{j}^{(\ell)}}{\sum_{j}\mu_{j}^{(\ell)}}, \, \forall i,j,\ell $.
This policy assigns servers proportional to their service rates. The choice of all parameters are then modifies to the closest norm feasible solution.  Using this initialization, the problem in \eqref{eq:joint_otp_prob} is optimized over the choice of $\boldsymbol{t}$, $\boldsymbol{b}$, $\boldsymbol{w}$, and $ \boldsymbol{p}$ (using Algorithms  \ref{alg:NOVA_Alg1},  \ref{alg:NOVA_Alg3},  \ref{alg:NOVA_Alg4}, and \ref{alg:NOVA_Alg5}, respectively)  using alternating minimization. 

%These access probabilities are projected toward feasible region to ensure
%stability of the storage system. With these fixed access probabilities,
%the joint quality-stall duration is optimized over the remaining four
%sets of variables: bandwidth allocation $\boldsymbol{w}$, quality
%probabilities $\boldsymbol{b}$, VMs selection probabilities $\boldsymbol{p}$, and the auxiliary variables $\boldsymbol{t}$.


%% 6
\item {\em Projected Lowest Quality, Optimized Bandwidth Wights, Auxiliary variables and Server Access (PLQ-BTA):}
In this strategy, we set
 $b_{i,1}=1\,\text{and \ensuremath{b_{i,\ell}=0},\ \ensuremath{\forall\ell}}\neq1$ in the initialization thus choosing the lowest quality for all videos.  Then, this choice is projected to the  closest norm feasible solution. Using this initialization, the problem in \eqref{eq:joint_otp_prob} is optimized over the choice of $\boldsymbol{q}$, $\boldsymbol{t}$, $\boldsymbol{w}$, and $ \boldsymbol{p}$  (using Algorithms  \ref{alg:NOVA_Alg1Pi}, \ref{alg:NOVA_Alg1},  \ref{alg:NOVA_Alg4}, and \ref{alg:NOVA_Alg5}, respectively)  using alternating minimization. 
 
 

%% 7
\item {\em Projected Highest Quality, Optimized Bandwidth Wights, Auxiliary variables and Server Access (PHQ-BTA):}  In this strategy, we set
$b_{i,6}=1\,\text{and \ensuremath{b_{i,\ell}=0},\ \ensuremath{\forall\ell}}\neq6$ in the initialization thus choosing the highest quality for all videos.  Then, this choice is projected to the  closest norm feasible solution. Using this initialization, the problem in \eqref{eq:joint_otp_prob} is optimized over the choice of $\boldsymbol{q}$, $\boldsymbol{t}$, $\boldsymbol{w}$, and $ \boldsymbol{p}$  (using Algorithms  \ref{alg:NOVA_Alg1Pi}, \ref{alg:NOVA_Alg1},  \ref{alg:NOVA_Alg4}, and \ref{alg:NOVA_Alg5}, respectively)  using alternating minimization. 

\end{enumerate} 



%\begin{figure*}[htb]
%	\centering
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\includegraphics[trim=0in 0in 0in 0.0in, clip, width=\textwidth]{figs/stallconvrg}
%		%	\vspace{-.3in}
%		\captionof{figure}{Convergence of mean stall duration.}
%		\label{fig:ConvgMeanStall}
%	\end{minipage}%
%	\hspace{2mm}
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\includegraphics[trim=0.0in 0in 0.0in 0in, clip, width=\textwidth]{figs/stall_vs_arrRate}
%		%	\vspace{-.3in}
%		\captionof{figure}{Mean stall duration for different video arrival rates with different video lengths. }
%		\label{fig:meanArrRateSameSize}
%	\end{minipage}
%	\hspace{2mm}
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\includegraphics[trim=0.0in 0in 0.0in 0in, clip,width=\textwidth]{figs/qlty_vs_arrRate}
%		%		\vspace{-.3in}
%		\captionof{figure}{Mean stall duration for different video sizes considering  $\ell=3$.  }
%		\label{fig:meanArrRateDiffSize}
%	\end{minipage}
%	%\vspace{-.2in}
%	
%	\vspace{-.1in}
%\end{figure*}


\subsection{Results}
In this subsection, we
set $\theta = 10^{-7}$, {\em i.e.}, prioritizing stall minimization over quality enhancement. We note that the average quality numbers are orders of magnitude higher than the mean stall duration and thus to bring the two to a comparable scale, the choice of $\theta = 10^{-7}$ is small.  This choice of $\theta$ is motivated since users prefer not seeing interruptions more than seeing better quality. 

%by the user preference of watching a smooth video with reduced quality over watching a better quality video with frequent interruptions.



%focus only on minimizing the mean stall duration of all files by setting $\theta=1$, {\em i.e.}, stall duration tail probability is not considered.% in this part of the simulation.

%\subsubsection*{Convergence of the Proposed Algorithm}
%Figure \ref{fig:ConvgMeanStall} shows the convergence  of our proposed algorithm, which alternatively optimizes the mean stall duration of all files over server scheduling probabilities $\boldsymbol{q}$, VMs selection access $\boldsymbol{p}$, auxiliary variables $\boldsymbol{t}$, quality probabilities $\boldsymbol{b}$, and bandwidth allocation weights $\boldsymbol{w}$. We notice that for $r=1000$ video files of size 600 sec with $m=12$ storage nodes and six quality levels shown in \ref{tab:DataRates}, the mean stall duration converges to the optimal value within less than $2100$ iterations.  
%
%
%\subsubsection*{Effect of Arrival Rate} Figures \ref{fig:meanArrRateSameSize}   and \ref{fig:meanArrRateQlty} show the effect of different video arrival rates on the mean stall duration and weighted averaged quality, respectively, for different-size video  whose lengths follow the Pareto-distributed described above.  We compare our proposed algorithm with the six baseline  policies and see that the proposed algorithm outperforms all baseline strategies for the QoE metrics of mean stall duration and weighted average quality. Thus, sever access, VMs selection and bandwidth weights allocation of files are important for the reduction of mean stall duration. While the mean stall duration increases with arrival, our approach still maintain low mean stall duration compared to the baselines. Moreover, we observe that the algorithms that optimize the quality tend to increase the quality of the streamed video only if the stall durations are zero (or close to zero) and adopt the lowest quality if the stall durations are not zero.
%Figure \ref{fig:meanArrRateQlty}
%shows that PLQ-BTA (PHQ-BTA) streaming policy realizes the lowest (highest) mean stall duration as it is aggressively minimize (maximize) the stall (quality) at the cost of quality (stall)-related-optimized parameters.



%While the PLQ-BTA (PHQ-BTA) algorithm achieves the highest quality, its performance in terms of stall is the worst as it is always biased to stream the video with the highest possible quality without optimizing thes


%Intuitively, having optimized placement leads to less stall duration (for all policies) since video chunks are balanced across the different storage nodes. Hence, the possibility of congested bottleneck nodes reduces accordingly. While mean stall duration increases as arrival rate increases, our approach, unlike PEAP and BNW, does not explode  as others do (especially for optimized one). 

%\subsubsection*{Effect of Video Size}
%The effect of having different video sizes is also captured in Figure (\ref{fig:meanArrRateDiffSize}). Clearly, larger video sizes may incur more stalls compared to small ones as the chance of getting delayed chunks is increased. However, our proposed approach gives the lowest mean stall duration compared to the considered baselines.
%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_7_mean_stall_NoOfFiles_source.eps}
%\caption{Mean stall duration for different number of video files with different video sizes. \label{fig:meanStallNumFiles} }
%\end{figure}


%\subsubsection*{Effect of the Number of Video Files}
%
%Figure \ref{fig:meanStallNumFiles} demonstrates the impact of varying the number of video files from $200$ files to $1000$ files  on the mean stall duration, where the video lengths are generated according to Pareto distribution with the same parameter defined earlier (scale of 300, and shape of 2).  We note that the proposed optimization strategy effectively reduces the mean stall duration and outperforms the considered baseline strategies. Thus, joint optimization over all three variables $\boldsymbol{t}$,  $\boldsymbol{\pi}$,  $\boldsymbol{w}$, and  $\boldsymbol{b}$ helps reduce the mean stall duration significantly.


%\subsection{Average Quality  Optimization}
%
%In this subsection, we consider optimizing (magnifying) the quality of the streamed video by maximizing the quality probabilities, $\boldsymbol{b}$, by setting $0.5\leq\theta_{q}\leq1$
% in (\ref{eq:joint_otp_prob}).

%\subsubsection*{Varying Quality factor parameter}
%Figure \ref{fig:congStallDiffXvalues} 
% shows the average quality of the streamed videos versus the
%stall factor $\theta_{s}$ for the selected set of algorithms. Apparently,
%our proposed approach gives the highest quality as it aggressively
%maximizes the quality over the stall duration, i.e., streaming the
%larger videos by the highest possible probability. These results show
%also the greedy behavior of our proposed approach as $\theta_{q}$  increases (or alternatively $\theta_{s}$ decreases) and clearly at $\theta_{q}=1$ (that is, $\theta_{s}=0$) our approach streams the video of the largest size and thus the average quality of the streamed video is
%$\ell=6$, i.e., which is the highest possible quality. 


%\begin{figure*}
%	\centering
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\includegraphics[trim=0.0in 0in 0.0in 0in, clip, width=\textwidth]{figs/stall_vs_vidlengh}
%%		\vspace{-.3in}
%		\captionof{figure}{Mean stall duration for different number of video files with different video lengths.}
%		\label{fig:meanStallNumFiles} 
%	\end{minipage}%
%	\hspace{2mm}
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\includegraphics[trim=0.0in 0in 0.0in 0in, clip, width=\textwidth]{figs/qlty_vs_vidlengh}
%%		\vspace{-.3in}
%		\captionof{figure}{ Average Streamed Quality versus quality factor $\theta_q$}
%		\label{fig:congStallDiffXvalues}
%	\end{minipage}
%	\hspace{2mm}
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\includegraphics[trim=0in 0in 0.1in 0in, clip,width=\textwidth]{figs/qlty_stall_vs_d_j}
%%		\vspace{-.3in}
%		\captionof{figure}{Average Video Quality and Mean Stall duration versus the number of virtual queues $d$}
%		\label{fig:tailProbDiffX}
%	\end{minipage}
%%	\vspace{-.2in}
%
%\vspace{-.15in}
%\end{figure*}




%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_8_stallTail_vs_Num_iterations_source2.eps}
%\caption{Stall duration Tail Probability for different $x$. \label{fig:congStallDiffXvalues} }
%\end{figure}

%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_9_wieghtedLat_vs_x_comp_logy_source.eps}
%\caption{Stall duration tail probability for different $x$ (in seconds). \label{fig:tailProbDiffX} }
%\end{figure}
%\subsubsection*{ Effect of the Number of the Virtual Queues $d$}
%Figure \ref{fig:tailProbDiffX} plots the 
%average of the streamed video quality and mean stall duration versus the number of virtual queses $d$. We vary the number of VQs from 5 to 30 with increment step of 5 and we set $\theta_q=1e-6$. We can see that the stall duration decreases as the number of VQs increases since more jobs can be handled simultaneously. We also observe that the proposed algorithm gives higher quality as $d$ increases which results from serving more than a job concurrently and allows for larger videos to be served. Hence, the proposed algorithm manages to significantly improve the two QoE metrics as $d$ increases.

%\begin{figure*}
%	\centering
%%	\begin{minipage}{.32\textwidth}
%%		\centering
%%		\includegraphics[trim=0in 0in 0.1in 0in, clip, width=\textwidth]{figs/tradeOff}
%%%		\vspace{-.3in}
%%		\captionof{figure}{Stall duration tail probability for different arrival rates for video files ($x=150$ s).}
%%		\label{fig:tailProbArrRate}
%%	\end{minipage}%
%%		\hspace{2mm}
%%		\begin{minipage}{.32\textwidth}
%%			\centering
%%		\includegraphics[trim=0in 0in 0.1in 0in, clip, width=\textwidth]{figs/convgstall2}
%%%		\vspace{-.3in}
%%		\captionof{figure}{Stall duration tail probability for varying number of video files ($x=150$ s).}
%%		\label{fig:Fig_9_stallLat_vs_NumOfFiles}
%%		\end{minipage}
%%		\hspace{2mm}
%		\begin{minipage}{.32\textwidth}
%			\centering
%			\includegraphics[trim=0in 0in 0.0in 0in, clip,width=\textwidth]{figs/tradeOff}
%	%		\vspace{-.3in}
%			\captionof{figure}{Tradeoff between mean stall duration and stall duration tail probability obtained by varying $\theta$.  }
%			\label{fig:tradeoff}
%		\end{minipage}
%	
%		\vspace{-.2in}
%\end{figure*}

%\begin{figure}[t]
%	\centering
%%		\hspace{2mm}
%		\begin{minipage}{.32\textwidth}
%			\centering
%			\includegraphics[trim=0in 0in 0.0in 0in, clip,width=\textwidth]{figs/tradeOff}
%	%		\vspace{-.3in}
%			\captionof{figure}{Tradeoff between mean stall duration and streamed video quality obtained by varying $\theta_s$.  }
%			\label{fig:tradeoff}
%		\end{minipage}
%	
%		\vspace{-.2in}
%\end{figure}


%\subsection{Tradeoff  between mean stall duration and video quality}
%
%
%The preceding results show a trade off between the mean stall duration and
%the streamed quality. In order to investigate such tradeoff, Figure \ref{fig:tradeoff} plots the average video quality versus the mean stall duration for different values of $\theta$ ranging from $\theta=10^{-5}$ to $\theta=10^{-7}$. This figure implies that a compromise between the two QoE metrics can be achieved by our proposed   streaming algorithm by setting the quality and stall factors ($\theta_q$ and $\theta_s$) to proper values. As expected, increasing $\theta_s$ will reduce the mean stall duration as higher priority is giving to minimize the stall over the quality. Thus, an efficient tradeoff point between the QoE metrics can be chosen based on the point on the curve that is appropriate for the clients.


\input{results}

==> sec_7_Appendx.tex <==
\section{Conclusion}
